The Last Mile: High-Assurance and High-Speed Cryptographic Implementations

We develop a new approach for building cryptographic implementations. Our approach goes the last mile and delivers assembly code that is provably functionally correct, protected against side-channels, and as efficient as hand-written assembly. We illustrate ur approach using ChaCha20-Poly1305, one of the mandatory ciphersuites in TLS 1.3, and deliver formally verified vectorized implementations which outperform the fastest non-verified code. We realize our approach by combining the Jasmin framework, which offers in a single language features of high-level and low-level programming, and the EasyCrypt proof assistant, which offers a versatile verification infrastructure that supports proofs of functional correctness and equivalence checking. Neither of these tools had been used for functional correctness before. Taken together, these infrastructures empower programmers to develop efficient and verified implementations by "game hopping", starting from reference implementations that are proved functionally correct against a specification, and gradually introducing program optimizations that are proved correct by equivalence checking. We also make several contributions of independent interest, including a new and extensible verified compiler for Jasmin, with a richer memory model and support for vectorized instructions, and a new embedding of Jasmin in EasyCrypt.

==> eqcheck_old.tex <==

\section{Source-level verification}
\label{sec:eqcheck}

This section describes our embedding of \Jasmin in \EasyCrypt. We use
this embedding for proving correctness of reference implementations,
equivalence between reference and optimized implementations, and
finally constant-time security of implementations.

\subsection{Design choices and issues}
Rather than building a verified verification infrastructure on top of
the \Coq formalization of the language (a la VST~\cite{Appel14}), we
opt for embedding \Jasmin into \EasyCrypt~\cite{BartheDGKSS13}, a
proof assistant for cryptographic proofs. We choose this route for
pragmatic reasons: \EasyCrypt already provides infrastructure for
functional correctness and relational proofs, and achieves good levels
of automation via backends to SMT-solvers. Moreover it provides good
support for provable security proofs (although it is not exploited in
this paper). On the other hand, embedding \Jasmin in \EasyCrypt leads
to duplicate work, since we must define an embedding of the \Jasmin
language into \EasyCrypt. Although we already have an encoding of
\Jasmin into \Coq, we cannot reuse this encoding for two reasons:
first, we intend to exploit maximally the verification infrastructure
of \EasyCrypt, so the encoding should be fine-tuned to achieve this
goal. Second, the \Coq encoding uses dependent types, which are not
available in \EasyCrypt. However, these are relatively simple issues
to resolve, and the amount of duplicate work is largely compensated by
the gains of using \EasyCrypt for program verification (also note that
building a verified verification infrastructure in \Coq requires some
effort).

\subsection{An overview of \EasyCrypt}

\subsection{Embedding \Jasmin in \EasyCrypt}
The native language of \EasyCrypt provides control-flow structures
that perfectly match those in \Jasmin, including {\sf if}, {\sf while}
and {\sf call} commands. This leaves us with two issues: 1) to encode
the semantics of all x86 instructions (including SIMD) in \EasyCrypt;
and 2) to encode the memory model of \Jasmin in \EasyCrypt.


\subsubsection*{Instruction semantics}
Our formalization of x86 instructions aims at being both readable and
amenable to building a library of reusable properties over the defined
operations, in particular over SIMD instructions.  The first step is
to define a generic theory for words of size $k$, with the usual
arithmetic and bit-wise operations. The semantics of arithmetic
operations are based on two injections (signed and unsigned) into
integers and arithmetic modulo $2^k$. For bit-wise operations, we rely
on an injection to Boolean arrays of size $k$.  Naturally a link
between both representations (int and Boolean array) is also created,
which allows proving for example that shifting a word $n << i$ is the
same as multiplying it by $\textsf{to\_uint}~ 2^i$.

Scalar x86 operations are formalized using the theory for words, and
useful lemmas about the semantics of these instructions are also
proved as auxilliary lemmans. For example, the formalizations of
\textsf{shl} and \textsf{shr} permit proving lemmas like
$\mathsf{shl}~x~i \oplus \textsf{shr}~x~(k - i) = \textsf{rol}~x~i$,
under appropriate conditions on $i$.

The semantics of SIMD instructions rely on the theories for 128/256
bit words, but the semantics must be further refined to enable viewing
words as arrays of sub-words, which may be nested (e.g., instruction
\textsf{vpshufd} sees 256-bit wordsas two 128-bit words, each of them
viewed as an array of sub-words).  To ease this kind of definition, we
have defined a bijection between words and arrays of (sub-)words of
various sizes.  Then vector instruction are defined in terms of arrays
of words.

\bg{Say something on generic lemma (rewrite rules) which considerably simplify the proof.}

\subsubsection*{Memory model}
\EasyCrypt does not provide the notion of pointer natively.
We rely on the concept of a global variable in \EasyCrypt, which can be modified by side effects of procedures, to emulate the global memory of \Jasmin and the concept of pointer to this memory.
A dedicated \EasyCrypt library defines abstract type \ec{global_mem_t} equipped with two basic operations for load \ec{mem.[p]} and store \ec{mem\.[p<-x]} of one byte, as follows:

{\begin{lstlisting}[language=easycrypt,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
type address = int.
type global_mem_t.
op "_.[_]" : global_mem_t -> address -> W8.t.
op "_.[_<-_]" : global_mem_t -> address -> W8.t -> global_mem_t.
axiom get_setE m x y w : m.[x <- w].[y] = if y = x then w else m.[y].
\end{lstlisting}}

From this basic axiom we build the semantics of load and store instructions
for various word sizes. The \Jasmin memory library then defines a single
global variable \ec{Glob.mem} of type \ec{global_mem_t}, which is accessible
to other \EasyCrypt modules and is used to express pre-conditions and 
post-conditions on memory states.

\paragraph*{Soundness}
\gb{needs to be rewritten}
We note that safety analysis also plays an important role in
the relation between the new \EasyCrypt axiomatic model of \Jasmin
semantics and the \Jasmin semantics as formalized in \Coq. Indeed,
these semantics match for safe programs, which gives meaning to
equivalence proofs between \Jasmin extracted code and specifications
written in \EasyCrypt, for which safety could mean a totally different
(for example, our specification of \poly performs pointer arithmetic
over the integers as can be seen in Figure~\ref{fig:polyspec}).
\mbb{Make sure poly spec is written this way.}

\subsection{Reusable multi-precision libraries}

-  o controle apertado sobre o “espaço vivo” nos registos (não sei bem como chamar a isso — live bits?, ou ou simplesmente range analysis). Aqui o interessante é que se devenvolveram teorias para o SMT que permitem resolver de forma automática a generalidade dos objectivos de prova resultantes (na verdade, isto é mais aplicável ao predicado “bW64” — já o “ubW64” não é bem assim, mas tenciono ainda voltar lá para melhorar um bocado a coisa…)
- na prova de correcção das operações aritméticas, parte do argumento está generalizado para representações com números arbitrários de limbs (como as operações de adição com propagação de carry, ou o alg. schoolbook multiplication; etc.). Tipicamente, o que fica específico em cada representação é a parte de redução modular, que normalmente acaba por ser tratado caso a caso.

\subsection{Verification of side-channel security}
\gb{I would move some material from section 2 here}



==> listings/chacha_hacl.tex <==
%!TEX root = ../main.tex

{\begin{lstlisting}[language=C,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
inline static void Hacl_Impl_Chacha20_quarter_round(
         uint32_t *st, uint32_t a, uint32_t b, 
         uint32_t c, uint32_t d)
{



  uint32_t sa = st[a];
  uint32_t sb0 = st[b];
  st[a] = sa + sb0;
  uint32_t sd = st[d];
  uint32_t sa10 = st[a];
  uint32_t sda = sd ^ sa10;
  st[d] = Hacl_Impl_Chacha20_rotate_left(sda, (uint32_t)16U);
  uint32_t sa0 = st[c];
  uint32_t sb1 = st[d];
  st[c] = sa0 + sb1;
  uint32_t sd0 = st[b];
  uint32_t sa11 = st[c];
  uint32_t sda0 = sd0 ^ sa11;
  st[b] = Hacl_Impl_Chacha20_rotate_left(sda0, (uint32_t)12U);
  ...

}

inline static void 
   Hacl_Impl_Chacha20_sum_states(uint32_t *st, uint32_t *st_)
{
  for (uint32_t i = (uint32_t)0U; i < (uint32_t)16U; 
                                                   i = i + (uint32_t)1U)
  {
    uint32_t xi = st[i];
    uint32_t yi = st_[i];
    st[i] = xi + yi;
  }
}
\end{lstlisting}}

==> listings/chacha_jasmin.tex <==
%!TEX root = ../main.tex



{\begin{lstlisting}[xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
fn Hacl_Impl_Chacha20_quarter_round(
     stack u32[16] st, inline int a, inline int b, 
     inline int c, inline int d) -> stack u32[16]
{
  reg u32 sa, sb0, sd, sa10, sda, sa0, sb1, sd0, sa11, 
  sda0, sa2, sb2, sd1, sa12, sda1, sa3, sb, sd2, sa1, sda2;

  sa = st[a];
  sb0 = st[b];
  sa += sb0;  st[a] = sa;
  sd = st[d];
  sa10 = st[a];
  sda = sd ^ sa10;
  st[d] = Hacl_Impl_Chacha20_rotate_left(sda, i_16);
  sa0 = st[c];
  sb1 = st[d];
  sa0 += sb1; st[c] = sa0;
  sd0 = st[b];
  sa11 = st[c];
  sda0 = sd0 ^ sa11;
  st[b] = Hacl_Impl_Chacha20_rotate_left(sda0, i_12);
  ...
  return st;
}

fn Hacl_Impl_Chacha20_sum_states(stack u32[16] st, 
                      stack u32[16] st_) -> stack u32[16]
{
  reg u32 xi, yi;
  inline int i;

  for i=0 to 16
  { xi = st[i]; yi = st_[i]; xi += yi; st[i] = xi; }
  return st;
}
\end{lstlisting}}

==> listings/gimliref.tex <==
%!TEX root = ../main.tex



{\begin{lstlisting}[language=easycrypt,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
inline fn gimli_body(stack u32[12] state) -> stack u32[12] {
   inline int round, column;
   reg u32 x, y, z;
   
   for round = 24 downto 0 {
     for column = 0 to 4 {              
        x = state[column];     x = rotate(x, 24);
        y = state[4 + column]; y = rotate(y, 9);
        z = state[8 + column];
  
        state[8 + column] = x ^ (z << 1) ^ ((y & z) << 2);
        state[4 + column] = y ^ x ^ ((x | z) << 1);
        state[column]     = z ^ y ^((x & y) << 3);
     }
     if (round % 4) == 0 { 
       x = state[0]; y = state[1];
       state[0] = y; state[1] = x;
       x = state[2]; y = state[3];
       state[2] = y; state[3] = x;
     }
     if (round % 4) == 2 { 
       x = state[0]; y = state[2];
       state[0] = y; state[2] = x;
       x = state[1]; y = state[3];
       state[1] = y; state[3] = x;
     }
     if (round % 4) == 0 {
       state[0] = state[0] ^ (0x9e377900 ^32u round);
     }      
   }
   return state;
}

\end{lstlisting}}


==> listings/poly1305_amd64_avx2.tex <==
%!TEX root = ../main.tex

{\begin{lstlisting}[xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
fn remaining_blocks(
  reg u128[5] hxy, reg u64 in, stack u128[5] s_r4r4, 
  stack u128[4] s_r4r4x5, stack u128[5] s_r2r2, 
  stack u128[4] s_r2r2x5) -> reg u128[5], reg u64
{
  reg u128[5] xy0, xy1;

  hxy = mulmod_u128(hxy, s_r4r4, s_r4r4x5);
  xy0 = unpack_u128x2_to_u26x5x2(in);
  in += 32;
  hxy = mulmod_add_u128(hxy, xy0, s_r2r2, s_r2r2x5);
  xy1 = unpack_u128x2_to_u26x5x2(in);
  in += 32;
  hxy = add_u128(hxy, xy1);
  hxy = carry_reduce_u128(hxy);
  return hxy, in;
}
\end{lstlisting}}

==> listings/poly1305_amd64_leaf.tex <==
%!TEX root = ../main.tex



{\begin{lstlisting}[xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
fn mulmod_add(reg u64[5] u, reg u64[5] x, 
    stack u64[5] y, stack u64[4] yx5) -> reg u64[5]
{
  reg u64[5] t;
  reg u64[3] z;

  t[0] = x[0]; t[0] *= y[0]; 
  t[1] = x[0]; t[1] *= y[1]; 
  t[2] = x[0]; t[2] *= y[2]; 
  t[3] = x[0]; t[3] *= y[3]; 
  t[4] = x[0]; t[4] *= y[4]; 
  ...
\end{lstlisting}}

==> listings/poly1305_amd64_leaf_avx2.tex <==
%!TEX root = ../main.tex

{\begin{lstlisting}[xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none]
fn mulmod_add_u128(reg u128[5] u, reg u128[5] x, 
    stack u128[5] y, stack u128[4] yx5) -> reg u128[5]
{
  reg u128[5] t, z, p;
  reg u128 c;

  t[0] = #x86_VPMULU(x[0], y[0]);
  t[1] = #x86_VPMULU(x[0], y[1]);
  t[2] = #x86_VPMULU(x[0], y[2]);
  t[3] = #x86_VPMULU(x[0], y[3]); 
  t[4] = #x86_VPMULU(x[0], y[4]);
  ...
\end{lstlisting}}

==> listings/poly1305_opt.tex <==
%!TEX root = ../main.tex



{\begin{lstlisting}[xleftmargin=0pt,xrightmargin=0pt,basicstyle=\footnotesize,frame=none, escapeinside={(*}{*)}]
fn carry_reduce_avx2(reg u256[5] x, reg u256 mask26) -> reg u256[5]
{
  reg u256[2] z;
  reg u256 t;

  z[0] = x[0] >>4u64 26;  (* \hspace{0.1cm} *) z[1] = x[3] >>4u64 26;
  x[0] &= mask26;         (* \hspace{0.1cm} *) x[3] &= mask26;
  x[1] +4u64= z[0];       (* \hspace{0.2cm} *) x[4] +4u64= z[1];
  z[0] = x[1] >>4u64 26;  (* \hspace{0.1cm} *) z[1] = x[4] >>4u64 26;
  
  t = z[1] <<4u64 2;      
  z[1] +4u64= t;  
  
  x[1] &= mask26;        (* \hspace{0.1cm} *) x[4] &= mask26;
  x[2] +4u64= z[0];      (* \hspace{0.2cm} *) x[0] +4u64= z[1];
  z[0] = x[2] >>4u64 26; (* \hspace{0.1cm} *) z[1] = x[0] >>4u64 26;
  x[2] &= mask26;        (* \hspace{0.1cm} *) x[0] &= mask26;
  x[3] +4u64= z[0];      (* \hspace{0.2cm} *) x[1] +4u64= z[1];
  
  z[0] = x[3] >>4u64 26;
  x[3] &= mask26;
  x[4] +4u64= z[0];

  return x;
}
\end{lstlisting}}

